A Deep-Learning Enhanced Gappy Proper Orthogonal Decomposition Method for Conjugate Heat Transfer Problem

The current study aims to develop a non-intrusive Reduced Order Model (ROM) to reconstruct the full temperature field for a large-scale industrial application based on both numerical and experimental datasets. The proposed approach is validated against a domestic refrigerator. At the full order level, air circulation and heat transfer in fluid and between fluid and surrounding solids in the fridge were numerically studied using the Conjugated Heat Transfer (CHT) method to explore both the natural and forced convection-based fridge model followed by a parametric study-based on the ambient temperature, fridge fan velocity, and evaporator temperature. The main novelty of the current work is the introduction of a stable Artificial Neural Network (ANN) enhanced Gappy Proper Orthogonal Decomposition (GPOD) method which shows better performance than the conventional GPOD approach in such large-scale industrial applications. The full-order model is validated with the experimental results and the prediction accuracy of the surrogate model associated with different reduced-order approaches is compared with the benchmark numerical results or high-fidelity results. In our current work, we show that a prediction error of one degree centigrade and computational speed-up of 5000 is achieved even at a very sparse training dataset using the proposed deep-learning enhanced GPOD approach.

==> Command.tex <==
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}

\def\a{{\bm a}}
\def\b{{\bm b}}
\def\d{{\bm d}}
\def\f{{\bm f}}
\def\g{{\bm g}}
\def\n{{\bm n}}
\def\u{{\bm u}}
\def\v{{\bm v}}
\def\w{{\bm w}}
\def\x{{\bm x}}
\def\P{{\bm P}}
\def\U{{\bm U}}
\def\X{{\bm X}}
\def\0{\boldsymbol{0}}
\def\ss{\boldsymbol{\sigma}}
\def\SS{\boldsymbol{\Sigma}}
\def\ee{\boldsymbol{\eta}}
\def\mubar{\overline{\mu}}
\def\ubar{\overline{\u}}
\def\vbar{\overline{\v}}
\def\vtilde{\tilde{\v}}
\def\wbar{\overline{\w}}
\def\qbar{\overline{q}}
\def\dt{\partial_t}
\def\bbf{\mathbf{b}}
\def\ebf{\mathbf{e}}
\def\fbf{\mathbf{f}}
\def\qbf{\mathbf{q}}
\def\pbf{\mathbf{p}}
\def\vbf{\mathbf{v}}
\def\ubf{\mathbf{u}}
\def\xbf{\mathbf{x}}
\def\ybf{\mathbf{y}}
\def\vbarbf{\overline{\vbf}}
\def\qbarbf{\overline{\qbf}}
\def\xbarbf{\overline{\xbf}}
\def\bbarbf{\overline{\bbf}}

\def\uh{\u_h}
\def\vh{\v_h}
\def\fh{\f_h}
\def\bh{\b_h}
\def\ph{p_h}
\def\qh{q_h}
\def\vbarh{\vbar_h}
\def\qbarh{\qbar_h}
\def\mubarh{\mubar_h}

\def\cl {\nonumber \\}
\def\el {\nonumber }

\newtheorem{rem}{Remark}[section]

\def\Jcp{J. Comp. Phys}
\def\Cmame{Comput. Methods Appl. Mech. Engrg.}
\def\Jmpa{J. Math. Pures Appl.}
\def\Mmmas{Math. Model Meth. Appl. Sci.}
\def\Siamsc{SIAM J. Sci. Comp.}

\newcommand{\bm}[1]{\mbox{\boldmath{$#1$}}}
\def\div{\nabla\cdot}
\def\grad{\nabla}
\def\grads{\grad^s}

%\topmargin      10mm 
%\evensidemargin 5mm \oddsidemargin  5mm
%\textwidth      150mm \textheight 200mm \frenchspacing \sloppy

%\def\baselinestretch{2} 

\newcommand{\anna}[2][cyan]{\emph{\textcolor{#1}{#2}}}
\newcommand{\rev}[2][red]{{\textcolor{#1}{#2}}}



% To quantify the ROM accuracy, all snapshots are reconstructed in time using ROM techniques and the $l^2$-norm relative error for each snapshot is computed considering again three different energy threshold as before.  We were interested to see the effect of Dataset Size, i.e. Train to Test Split Ratios in our comparison to check the error convergence with the respect to this ratio. To this aim three ratio were considered; in the first case 50$\%$ of dataset is used to train the model, then 70$\%$ and finally 90$\%$ each of them for three various energy threshold.     

==> noncitebib.tex <==












@book{quarteroni2015reduced,
  title={Reduced basis methods for partial differential equations: an introduction},
  author={Quarteroni, A. and Manzoni, A. and Negri, F.},
  volume={92},
  year={2015},
  publisher={Springer}
}








%%%%%%%%5555 golshan
@article{review,
  title={Review and Implementation of CFD-DEM Applied to Chemical Process Systems},
  author={Golshan, S. and Sotudeh-Gharebagh, R. and Zarghami, R. and Mostoufi, N. and  Blais, B. },
  journal={ Chemical Engineering Science },
  year={2020}
}
%clayton
@manual{multi,
  title={Multiphase Flows with Droplets and Particles},
  author={Crowe, C.T. and Schwarzkopf, J.D. and Sommerfeld, M. and Tsuji, Y.},
  year={2012}
}

@article{tsu,
  title={Discrete particle simulation of two-dimensional fluidized bed.},
  author={Tsuji, Y. and Kawaguchi, T. and Tanaka, T.},
  volume={77},
  journal={Powder Technol.},
  pages={79-87},
  year={1993}
}

@article{Xu,
  title={Numerical simulation of the gas-solid flow in a fluidized bed by combining discrete particle method with computational fluid dynamics.},
  author={Xu, B. H. and Yu, A. B.},
  volume={52},
  journal={Chemical Engineering Science},
  pages={2785–2809},
  year={1997}
}

@manual{multi,
  title={Multiphase Flows with Droplets and Particles},
  author={Crowe, C.T. and Schwarzkopf, J.D. and Sommerfeld, M. and Tsuji, Y.},
  year={2012}
}




@article{heat,
  title={CFD-DEM simulation of heat transfer in fluidized beds: Model verification, validation, and application},
  author={Wang, S. and Luo, K. and Hu, C. and Lin, J. and Fan, J.},
  journal={Chemical Engineering Science},
  volume={197},
  pages={280-295},
  year={2019}
}

@article{review,
  title={Review and Implementation of CFD-DEM Applied to Chemical Process Systems},
  author={Golshan, S. and Sotudeh-Gharebagh, R. and Zarghami, R. and Mostoufi, N. and  Blais, B. },
  journal={ Chemical Engineering Science },
  year={2020}
}


%validation




%%%%%%%%%%%%

@manual{foam,
  title={Openfoam user guide},
  author={Greenshields, C. J.},
  year={2016}
}

@manual{liggghts,
  title={https://www.cfdem.com/media/DEM/docu/Section_intro.html},
  author={Kloss, C.}
}

@manual{rans,
  title={RANS Simulations using OpenFOAM Software},
  author={Jones, D. A. and Chapuis, M. and Liefvendahl, M. and Norrison, D. and Widjaja, R.},
  year={2016}
}

@mastersthesis{fantin,
  title={CFD-DEM Coupling for Systems of Fluid and Non-Spherical Particles},
  author={Fantin, D.},
  year={2018},
  school={TU Delft}
}


@article{menter,
  title={Ten years of industrial experience with the sst turbulence model.},
  author={Menter, F. R. and Kuntz, M. and Langty, R.},
  journal={Turbulence, heat and mass transfer},
  volume={4},
  pages={625-632},
  year={2003}
}

@article{li,
  title={A computational investigation of transient heat transfer in pneumatic transport of granular particles.},
  author={Li, J. and Mason, D. J. },
  journal={Powder Technol.},
   volume={112},
  pages={273–282},
  year={2000}
}









%%%%%%%%%%%%
@article{patil,
  title={Comparison of CFD-DEM heat transfer simulations with infrared/visual measurements},
  author={Patil, A. V. and Peters, E. A. J. F. and Kuipers, J. A. M.},
  journal={Chem. Eng. J.},
  volume={277},
  pages={388–401},
  year={2015}
}

@mastersthesis{fois,
  title={CFD modeling of gas-solid fluidized beds in OpenFOAM: a comparison between the Eulerian-Eulerian and Eulerian-Lagrangian methods},
  author={Fois, L. and Fatti, V.},
  year={2021},
  school={Politecnico di Milano}
}

%Liu, T., Han, D., Wang, J., Johnson, M.R., 2012. Effects of septal deviation on the airflow characteristics: using computational fluid dynamics models. Acta Otolaryngol. 132, 290–298.




@article{tsuji,
  title={Lagrangian numerical simulation
of plug flow of cohesionless particles in a horizontal pipe},
  author={Tsuji, Y. and Tanaka, T. and Ishida, T.},
  journal={Powder Technol.},
  volume={71(3)},
  pages={239–250},
  year={1992}
}

@article{shafer,
  title={Force schemes in simulation of granular material},
  author={Shäfer, J. and Dippel, S. and Wolf, D. E.},
  journal={ J. de Phys. I France},
  volume={6(1)},
  pages={5–20},
  year={1996}
}

@article{deen,
  title={Review of discrete particle modeling of fluidized beds},
  author={Deen, N. G. and Van Sint Annaland, M. and Van der Hoef, M. A. and Kuipers, J. A. M.},
  journal={Chem. Eng. Sci.},
  volume={62},
  pages={28–44},
  year={2007}
}

@article{hertz,
  title={Über die berührung fester elastischer körper (on the contact of elastic solids.)},
  author={Hertz, H.},
  journal={J. Reine und Angew. Math},
  volume={92},
  pages={156–171},
  year={1882}
}

@article{issa,
  title={Solution of the implicitly discretized fluid flow equations by Coupled CFD-DEM modeling: formulation, implementation and application to multiphase flowsoperator-splitting},
  author={Issa, R.I.},
  journal={J. Comput. Phys.},
  volume={62},
  pages={40–65},
  year={1986}
}

@article{macphe,
  title={Particle tracking in unstructured, arbitrary polyhedral meshes for use in CFD and molecular dynamics},
  author={Macpherson, G. B. and Nordin, N. and Weller, H. G.},
  journal={Commun. Numer. Methods Eng},
  volume={25},
  pages={263– 273},
  year={2009}
}

@article{su,
  title={Discrete element simulation of particle flow in arbitrarily complex geometries},
  author={Su, J. and Gu, Z. and Xu, X. Y.},
  journal={Chem. Eng. Sci.},
  volume={66},
  pages={6069–6088},
  year={2011}
}


@phdthesis{jasak,
  title={Error analysis and estimation for the finite volume method with applications to fluid flows},
  author={Fois, L. and Fatti, V.},
  year={1996},
  school={Imperial College}
}




@article{palacios,
  title={Proper-orthogonal decomposition of spatio-temporal patterns in fluidized beds},
  author={Cizmas, P. G. and Palacios, A. and O’Brien, T. and Syamlal, M.},
  journal={Chemical Engineering Science},
  volume={58},
  pages={4417-4427},
  year={2003}
}


@article{wallin,
  title={Data-driven model order reduction for granular media},
  author={Wallin, E. and Servin, M.},
  journal={Computational Particle Mechanics},
  volume={9},
  pages={15–28},
  year={2022}
}


@article{fani,
  title={Reduced-order discrete element method modeling},
  author={Boukouvala, F. and Gao, Y. and Muzzio, F. and Ierapetritou, M. G.},
  journal={Chemical Engineering Science},
  volume={95},
  pages={12-26},
  year={2013}Coupled CFD-DEM modeling: formulation, implementation and application to multiphase flows
}

@article{shuo,
  title={Development of a reduced-order model for large-scale {{E}}ulerian–{{L}}agrangian simulations},
  author={Li, S. and Duan, G. and Sakai, M.},
  journal={Advanced Powder Technology},
  volume={33},
  year={2022}
}


@article{shuo2,
  title={POD-based identification approach for powder mixing mechanism in Eulerian–Lagrangian simulations},
  author={Li, S. and Duan, G. and Sakai, M.},
  journal={Advanced Powder Technology},
  volume={33},
  year={2022}
}

@article{mori,
  title={Development of a robust {{E}}ulerian–{{L}}agrangian model for the simulation of an industrial solid–fluid system},
  author={Mori, Y. and Sakai, M.},
  journal={Chemical Engineering Journal},
  volume={406},
  year={2021}
}





@article{hajisharifi2021particle,
  title={Particle capture by drops in turbulent flow},
  author={Hajisharifi, A. and Marchioli, C. and Soldati, A.},
  journal={Physical Review Fluids},
  volume={6},
  number={2},
  pages={024303},
  year={2021},
  publisher={APS}
}

@article{hajisharifi2022interface,
  title={Interface topology and evolution of particle patterns on deformable drops in turbulence},
  author={Hajisharifi, A. and Marchioli, C. and Soldati, A.},
  journal={Journal of Fluid Mechanics},
  volume={933},
  year={2022},
  publisher={Cambridge University Press}
}

@book{clayton,
  title={Multiphase Flows with Droplets and Particles},
  author={Crowe, C. T. and Schwarzkopf, J. D. and Sommerfeld, M. and Tsuji, Y.},
  publisher={CRC Press},
  number={2},
  year={2011}
}







%%%% cite{fernandes} already exists!
%@article{fernandes2018validation,
%  title={Validation of the CFD-DPM solver DPMFoam in $$$\backslash$hbox $\{$OpenFOAM$\}$\^{}$\backslash$circledR $$ OpenFOAM{\textregistered} through analytical, numerical and experimental comparisons},
%  author={Fernandes, C and Semyonov, D and Ferr{\'a}s, LL and N{\'o}brega, J Miguel},
%  journal={Granular Matter},
%  volume={20},
%  number={4},
%  pages={1--18},
%  year={2018},
%  publisher={Springer}
%}

@misc{macher2006pharmaceutical,
  title={Pharmaceutical Industry Wastes $50$ Billion a Year due to Inefficient Manufacturing},
  author={Macher, J. and Nickerson, J.},
  year={2006},
  publisher={McDonough School of Business, Georgetown University, Washington, DC}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%
%ROM papers -introduction
@book{hesthaven2016certified,
  title={Certified reduced basis methods for parametrized partial differential equations},
  author={Hesthaven, J. S. and Rozza, G. and Stamm, B.},
  volume={590},
  year={2016},
  publisher={Springer}
}

@book{quarteroni2015reduced,
  title={Reduced basis methods for partial differential equations: an introduction},
  author={Quarteroni, A. and Manzoni, A. and Negri, F.},
  volume={92},
  year={2015},
  publisher={Springer}
}

@article{benner2015survey,
  title={A survey of projection-based model reduction methods for parametric dynamical systems},
  author={Benner, P. and Gugercin, S. and Willcox, K.},
  journal={SIAM review},
  volume={57},
  number={4},
  pages={483--531},
  year={2015},
  publisher={SIAM}
}

@misc{benner2017model,
  title={Model Reduction of Parametrized Systems., volume 1st ed. 2017 of MS\&A series},
  author={Benner, P. and Ohlberger, M. and Patera, A. and Rozza, G. and Urban, K.},
  year={2017},
  publisher={Springer}
}

@book{benner2021system,
  title={System-and Data-Driven Methods and Algorithms},
  author={Benner, P. and Grivet-Talocia, S. and Quarteroni, A. and Rozza, G. and Schilders, W. and Silveira, L. M. },
  year={2021},
  publisher={De Gruyter}
}


@article{bader,
  title={Certified Reduced Basis Methods for Parametrized Distributed Elliptic Optimal Control Problems with Control Constraints.},
  author={Bader, E. and Kärcher, M. and Grepl, M. A. and Veroy, K.},
  journal={SIAM Journal on Scientific Computing},
  volume={38},
  pages={A3921–A3946},
  year={2016}
}

@article{yuan2005reduced,
  title={A reduced-order model for a bubbling fluidized bed based on proper orthogonal decomposition},
  author={Yuan, T. and Cizmas, P. G. and O’Brien, T.},
  journal={Computers \& chemical engineering},
  volume={30},
  number={2},
  pages={243--259},
  year={2005},
  publisher={Elsevier}
}




%%%%%%%%%%
%POD works in industry





@article{dolci2016proper,
  title={Proper orthogonal decomposition as surrogate model for aerodynamic optimization},
  author={Dolci, V. and Arina, R.},
  journal={International Journal of Aerospace Engineering},
  volume={2016},
  year={2016},
  publisher={Hindawi}
}



@article{di2021coarse,
  title={Coarse-grain dem modelling in fluidized bed simulation: A review},
  author={Di Renzo, A. and Napolitano, E. S. and Di Maio, F.},
  journal={Processes},
  volume={9},
  number={2},
  pages={279},
  year={2021},
  publisher={MDPI}
}

%@article{piso,
%  title={Solution of the implicitly discretised fluid flow equations by operator-splitting},
%  author={Issa, R. I.},
%  journal={Journal of Computational Physics},
%   volume={62},
%  pages={40–65},
%  year={1986}
%}


==> sections/ROM.tex <==
\section{The reduced order model}\label{sec:ROM}
%\textcolor{red}{Qui scriviamo un preambolo. Prendere ispirazione dal paper LVAD.}\\
We assume that any Eulerian (Lagrangian) variable can be approximated as a linear combination of a certain number of basis functions depending on the space $\bm{x}$ (label $l$ identifying the particles) only, multiplied by scalar coefficients that depend on the time and/or parameters of the problem at hand which can be physical or geometrical. 

In this work, we are going to reconstruct the time evolution of the system and to consider the Stokes number $Stk$ (see eq. \ref{Stk}) as a parameter. %we consider the time and the Stokes number as parameters. 
For what concerns the Eulerian phase, we are interested in the reconstruction of the fluid volume fraction $\epsilon$ whilst for the Lagrangian phase we consider the position $\widetilde{\bm{x}}$
 %$(\widetilde{X}, \widetilde{Y}, \widetilde{Z})$ a
and the velocity $\widetilde{\u}$ of the particles.
Hence,
the variables $(\epsilon, \widetilde{\bm{x}},  \widetilde{\bm{u}})$ %to eqs. \textcolor{red}{add refs} 
are approximated by the reduced ones $(\epsilon_r, \widetilde{\bm{x}}_r,  \widetilde{\bm{u}}_r)$ as follows %\textcolor{red}{da modificare il prosieguo}

\begin{align}
\epsilon \approx \epsilon_r = \sum_{i=1}^{N_{\epsilon}^r} \bm{\alpha}_i(t, \bm{\pi}) {\varphi}_i(\bm{x}), \quad 
\bm{\widetilde{x}} \approx \bm{\widetilde{x}}_r = \sum_{i=1}^{N_{\widetilde{x}}^r} \bm{\beta}_i(t, \bm{\pi}) \bm{\xi}_i(l), \quad 
\bm{\widetilde{u}} \approx \bm{\widetilde{u}}_r = \sum_{i=1}^{N_{\widetilde{u}}^r} \bm{\gamma}_i(t, \bm{\pi}) \bm{\zeta}_i(l).\label{eq:ROM_1} %\\
%\u \approx \u_r = \sum_{i=1}^{N_u^r} \overline{\beta_i}(\bm{\pi}, t) \bm{\overline{\varphi}}_i(\bm{x}), \quad
%\overline{q} \approx \overline{q}_r = \sum_{i=1}^{N_{\overline{q}}^r} \overline{\gamma_i}(\bm{\pi}, t) \overline{\psi}_i(\bm{x}). \label{eq:ROM_2}
\end{align}

In \eqref{eq:ROM_1}, $N_{\Phi}^r$ denotes the cardinality of a reduced basis for the space field $\Phi$ = $\{\epsilon, \widetilde{\bm{x}},  \widetilde{\bm{u}}\}$ and $\bm{\pi}$ is the parameter vector (that for the problem at hand it coincides with the Stokes number $Stk$). 
%Here, we are interested in the time reconstruction of the flow field with no other parameter. 
%We remark that we consider different coefficients for the approximation of the potential vorticity $q$ and stream function $\psi$ fields. 
%q ≈ qr =
%N r
%q
%∑
%i=1
%βi(t)φi(x), ψ ≈ ψr =
%N r
%ψ
%∑
%i=1
%γi(t)ξi(x).(17)
%In (17), N r
%Φ denotes the cardinality of a reduced basis for the space field Φ = {q, ψ}. We remark
%that we consider different coefficients for the approximation of the potential vorticity q and stream
%function ψ fields. 

The proper orthogonal decomposition with interpolation (PODI) \cite{bui} % is the reduced order model adopted in the present work. 
has been widely adopted for the development of ROM not only in industrial contexts \cite{demo1, demo2019complete, demo2018efficient, salmoiraghi2018free, dolci2016proper, shah2022finite} %\textcolor{red}{prendiamo le citazioni riportate in  LVAD più quella con Nirav} %Several examples of applications based on PODI technique can be found in literature ranging 
%naval \textcolor{red}{citazioni paper LVAD}, automotive \textcolor{red}{citazioni paper LVAD}, and aeronautics \textcolor{red}{citazioni paper LVAD} \textcolor{red}{in generale citerei anche il lavoro con Nirav e qualcuno del gruppo (da decidere chi)} 
but also in biomedical engineering \cite{lvad, siena2022fast, pier, siena2022data}. It has been also used within a CFD-DEM framework but only for the time reconstruction \cite{shuo, shuo2, mori}. Here we consider two variants of the PODI approach: the global PODI and the local PODI. Both techniques have been employed in the Python package EZyRB \cite{demo2018ezyrb}. 

\subsection{POD with Interpolation}
%A global POD basis space is computed by time dependent FOM snapshots associated to sample points in the parameter space. 

The global PODI method is based on the following \emph{offline}-\emph{online} paradigm: %\textcolor{red}{da rivedere} %computationally expensive FOM simulations are carried out on powerful computational facilities
%during the offline phase for certain values of the parameter vector $\bm{\pi}$ whilst computationally cheap calculations for every new parameter vector instance are run on any device during the online phase. More specifically:

\begin{itemize}
\item during the offline phase: a set of time-dependent high-fidelity solutions is collected for a wide range of parameter values and a global reduced basis for the space of the reduced solutions is extracted
via POD. In this stage, the interpolation %\textcolor{red}{modificare se facciamo anche NN}
is performed in order to establish the relationship between time and parameters, and coefficients of the reduced solutions (modal
coefficients). Due to the large number of degrees of freedom, the offline phase is computationally expensive. However, it is carried out only once.
\item during the online phase: the modal coefficients for every new time and parameter instance are quickly obtained from the interpolation model. %\textcolor{red}{modificare se facciamo anche NN}. 
The reduced solution is given by the linear
combination of the reduced basis functions with the modal coefficients as weights (see eq. \eqref{eq:ROM_1}). %The
%computational cost of the online phase is much smaller than the cost of the offline phase.
\end{itemize}

Next, we are going to describe the building blocks of the above algorithm. Let $\Phi (t^i, \bm{\pi}^j)$ with $i = 1, \dots, N_t$ and $j = 1, \dots, N_k$ be the full order solutions obtained for different time instants $t^i$ and values of the parameter vector $\bm{\pi}^j$. Then we detect $N_s = N_t \cdot N_k$ input-output pairs $\{(t^i, \bm{\pi}^j), \Phi (t^i, \bm{\pi}^j)\}$ and we collect the snapshots in the matrix $\mathbb{\bm{S}} = [\Phi(t^1, \bm{\pi}^1), \dots, \Phi(t^{N_t}, \bm{\pi}^{N_k})]$. The application of the singular value decomposition to the matrix $\mathbb{\bm{S}}$ provides:\\
    \begin{equation}
    \mathbb{\bm{S}} = \U \bm{\Sigma} \bm{V}^T,
    \end{equation}
    where $\U \in \mathbb R^{{N_c}\times {N_s}}$ and $\bm{V} \in R^{{N_s}\times {N_s}}$ are the matrices composed by the left singular vectors  and right singular vectors, respectively, whilst $\bm{\Sigma} \in \mathbb R ^{{N_c}\times {N_s}}$ is the diagonal matrix containing the eigenvalues $\sigma_i$. %, and $\mathbf V \in R^{{N_s}\times {N_s}}$ is the matrix composed by the right-singular vectors. %with the symbol $^T$ denotes the transpose operation. 
    %The left singular vectors, namely the columns of $\U = [\phi_1, \phi_2, . . . , \phi_{N_s}]$, are the POD modes. 
    We are going to compute %to approximate the high-fidelity snapshots (i.e. the columns of \mathbb{\bm{S}}) by means of 
    $N_\Phi^r << N_s $ modes by minimizing the distance between the snapshots and their projection onto the space spanned by the reduced basis itself, i.e.:\\
    \begin{equation}
    argmin_{\U_{N_\Phi^r}} \| \mathbf\mathbb \mathbb{\bm{S}} - \U_{N_\Phi^r} \U_{N_\Phi^r}^T \mathbf\mathbb \mathbb{\bm{S}} \|_F \quad \text{with} \quad \U_{N_\Phi^r}^T\U_{N_\Phi^r} = \bm{I},
    \label{mode1}
    \end{equation}
where $\| \|_F$ is the Frobenius norm and $\U_{N_\Phi^r}$ is the matrix $\U$ truncated to the first $N_\Phi^r$ columns representing our POD space. %Therefore, the reduced basis of dimension $N_\Phi^r$ is the orthonormal set of vectors that minimizes the distance between the snapshots and their projection onto the space spanned by the 276 reduced basis itself.
    %where $\|\bullet\|$ is the Frobenius norm, $\U_k \in  \mathbb R ^{N_c \times k}$ and \textbf I is the identity matrix. 
    %Therefore, the reduced basis of dimension k is the orthonormal (with respect to the Euclidean norm) set of vectors that minimizes the distance between the snapshots and their projection onto the space spanned by the reduced basis itself.
    
     %In addition, the truncation error %committed %by retaining only $columns of $\U_k $ 
     %is given by the sum of the squares of the neglected singular values:\\
    %\begin{equation}
    %\sum_{i=N_\Phi^r+1}^{N_s}} \sigma_i^2
    %\end{equation}
    %Hence, the snapshot matrix \textbf S can be approximated with arbitrary accuracy by controlling the size k. Since the error is strictly related to the magnitude of the singular values, it's common setting $k$ equal to the smallest integer $\overline{k}$ such that:
Typically, the value of $N_\Phi^r$ is commonly chosen to meet a user-provided threshold $\delta$ for the cumulative
energy of the eigenvalues:
    \begin{equation}
    \frac{\sum_{i=1}^{N_\Phi^r}\sigma_i^2}{\sum_{i=1}^{N_s}\sigma_i^2} \ge \delta,
    \label{k_equation}
    \end{equation}
    %where $\epsilon$ is an arbitrary tolerance and the left hand side of \eqref{k_equation} is the relative information content of the POD basis, namely the percentage of energy of the snapshots (or cumulative energy of the eigenvalues) retained by the first $\overline{k}$ modes.\\
    %After constructing the POD space, we express the input snapshots as a linear combination of the POD modes:\\
    %\begin{equation}
    %\sum_{j=1}^{N_s} \alpha_j (\pi_i) \phi_j \approx \sum_{j=1}^{k}\alpha_j (\pi_i) \phi_j, \quad \quad \forall i \in [1, ..., N_s]
    %\end{equation}
After constructing the POD space, we can approximate the input snapshots by using eq. \eqref{eq:ROM_1}:\\
    \begin{equation}
    \Phi(t^i, \bm{\pi}^j) \approx \sum_{L=1}^{N_\Phi^r}\chi_L (t^i, \bm{\pi}^j) \phi_L, \quad \text{with} \quad i = 1, \dots, N_t \quad \text{and} \quad j = 1, \dots, N_k, 
    \end{equation}
    where the modal coefficients $\chi_L (t^i, \bm{\pi}^j)$ are the elements of the matrix $\bm{C} = \U_{N_{\Phi}^r}^T \bm{S} \in \mathbb{R}^{N_\Phi^r \times N_s}$. Then the ROM is built using as input-output data the pairs $\{(t^i, \bm{\pi}^j), \chi_L(t^i, \bm{\pi}^j)\}$ associated to the $L$-th POD mode $\phi_L$ with $L = 1, \dots, N_\Phi^r$, i.e. we impose that 

\begin{equation}
    \mathbb{A}_L(t^i, \bm{\pi}^j) = \chi_L(t^i, \bm{\pi}^j), %\quad \text{with} \quad i = 1, \dots, N_t \quad j = 1, \dots, N_k,
    \label{Al_2}
    \end{equation}
where 

 \begin{equation}
    \mathbb{A}_L(t^i, \bm{\pi}^j) = \sum_{m=1}^{N_t} \sum_{n=1}^{N_k} w_{L,m,n} \zeta_{L,m,n}(\| (t^i, \bm{\pi}^j) - (t^m, \bm{\pi}^n) \|). %\quad \for \quad L = 1, 2, ..., k
    \label{Al}
    \end{equation}

    
    %The interpolation of the modal coefficients $\chi_L(\bm{\pi}_i)$ is based on Radial Basis Functions \textcolor{red}{mettere referenza RBF, la trovi sempre nel paper LVAD}. As it will be explained further below, during the online phase of the method, for any new value of the parameter vector $\pi^*$, an approximation $\mathbb{A}_L(\pi^*) \approx \alpha_L(\pi^*)$ of the L-th modal coefficient yields as follows:\\
   
    Here $\zeta_{L,m,n}$ are the Radial Basis Functions \cite{buhmann2003radial}, %\textcolor{red}{inserire citazione RBF, prendila da LVAD},
    which we chose as Gaussian functions centered in $(t^m, \bm{\pi}^n)$ %, and $\|\bullet\|$ \textcolor{red}{denotes the Euclidean norm in $\mathbb{R}^P$} 
    and $w_{L,m,n} \in \mathbb{R}^{N_s}$ are unkown weights. Eq. \eqref{Al} can be %are computed so that the following interpolation property (based on the available input-output data $(\pi_i, \alpha_L(\pi_i))$) holds\\
    %\begin{equation}
    %\mathbb{A}_L(\pi^*) = \alpha_L(\pi_i), \quad \for \quad i = 1, 2, ..., N_s
    %\label{Al_2}
    %\end{equation}
    %By inserting Eq.\eqref{Al} into Eq.\eqref{Al_2} yields\\
    %\begin{equation}
    %\mathbb{A}_L(\pi^*) = \sum_{j=1}^{N_s} \omega_{L,j} \zeta_{L,j} (\| \pi^* - \pi_j \|_{\mathbb{R}^P}) = \alpha_L(\pi_i), \quad \for \quad i = 1, 2, ..., N_s
    %\end{equation}
     reformulated in terms of a  linear system\\
    \begin{equation}
    \bm{Z}_L \bm{w}_L = \bm{\chi}_L, %(\bm{\pi}_i)
    \label{sys}
    \end{equation}
    %where $\bm{Z}_L \in \mathbb{R}^{N_s \times N_s}$ %and $\chi_L \in \mathbb{R}^{N_s}$ 
    %is assembled as\\
    %\begin{equation}
    %[Z_L]_{ij} = \zeta_{L,m,n} (\| (t^i, \bm{\pi}^j) - (t^m, \bm{\pi}^n) \|)%, \quad \quad [\chi_L]_i= \chi_L(\bm{\pi}_i), \quad \quad i,j = 1, 2, ..., N_s.
    %\end{equation} 
    %and $\omega_L \in \mathbb{R}^{N_s}$ collects the unknown weights. 
    to be solved to obtain the weights $\bm{w}_L$ for every value of $L = 1, \dots, N_\Phi^r$ once at all in the offline phase.\\
Then, in the online phase, for any new pair time-parameter $(t^\star, \bm{\pi}^\star)$, the approximated modal coefficients $\mathbb{A}_L(t^\star, \bm{\pi}^\star)$ are calculated from eq. \eqref{Al} and the ROM solution is computed as:\\
    \begin{equation}
    \Phi_r(t^\star, \bm{\pi}^*) = \sum_{L=1}^{N_\Phi^r} \mathbb{A}_L(t^\star, \bm{\pi}^\star)\phi_L.               
    \end{equation} 

\subsection{Gappy POD}

The Gappy POD approach computes the temperature  field which is termed as missing or "gappy" data based on temperature sensor data available at a few sensor locations. A brief description of the Gappy POD approach is described as follows,

First, a mask matrix is developed to locate the rows where the data is available. For the temperature field prediction, the corresponding mask vector $n^{k}$ is as follows:

\begin{equation}
\label{eq_mask}
\begin{aligned}
& n^k = 0 \ \ \text{if} \ \ {U_i}^k \ \ \text{is missing},\\
& n^k = 1 \ \ \text{if} \ \ {U_i}^k \ \ \text{is known},\\
\end{aligned}
\end{equation}

where, ${U_i}^k$ denotes the $i^{th}$ element of the vector $U^{k}$, pointwise multiplication is defined as $(n^k,U^k)_{i}= {n_i}^k{U_i}^k$. The gappy inner product and induced norm can be expressed respectively as follows: 

\begin{equation}
\label{eq_mask}
\begin{aligned}
& (u,v)_{n} = ((n,u),(n,v)),\\
& (\Vert v \Vert)^2 = (v,v)_{n}
\end{aligned}
\end{equation}

Now, if the standard POD basis vector is defined as ${\phi}^k$ for the known snapshots set ${U^k}$ where $k = 1 \ \ \text{to} \ \ m$, let's assume g to be another solution vector where only sparse sensor data sets are available. Assuming that the solution vector $g$ lies among the snapshots where all the elements of the entire vector are known.$\Tilde{g}$ is the 


\subsection{Deep Learning Enhanced Gappy POD}



